Pangolin: An Efficient and Flexible Graph Pattern Mining System on CPU and GPU

There is growing interest in graph pattern mining (GPM) problems such as motif counting. GPM systems have been developed to provide unified interfaces for programming algorithms for these problems and for running them on parallel systems. However, existing systems may take hours to mine even simple patterns in moderate-sized graphs, which significantly limits their real-world usability. We present Pangolin, a high-performance and flexible in-memory GPM framework targeting shared-memory CPUs and GPUs. Pangolin is the first GPM system that provides high-level abstractions for GPU processing. It provides a simple programming interface based on the extend-reduce-filter model, which enables users to specify application-specific knowledge for search space pruning and isomorphism test elimination. We describe novel optimizations that exploit locality, reduce memory consumption, and mitigate the overheads of dynamic memory allocation and synchronization. Evaluation on a 28-core CPU demonstrates that Pangolin outperforms existing GPM frameworks Arabesque, RStream, and Fractal by 49x, 88x, and 80x on average, respectively. Acceleration on a V100 GPU further improves performance of Pangolin by 15x on average. Compared to state-of-the-art hand-optimized GPM applications, Pangolin provides competitive performance with less programming effort.

==> sections/tbl_3fsm.tex <==
\begin{table}[t]
\footnotesize
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|rr|rr|rr|rr}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Mico} & \multicolumn{2}{c|}{Patent} & \multicolumn{2}{c|}{Youtube} & \multicolumn{2}{c}{PDB}         \\ \hline
$sup$ & PA  & DG   & PA   & DG   & PA    & DG & PA    & DG \\ \hline
300   & 3.9 & 52.2 & 14.7 & 19.9 & 96.9  & -  & 63.7 & 281.4 \\
500   & 3.6 & 52.9 & 15.8 & 18.7 & 97.7  & -  & 65.6 & 279.5 \\
1000  & 3.0 & 59.1 & 18.1 & 18.6 & 98.0  & -  & 73.4 & 274.5 \\
5000  & 2.4 & 58.1 & 27.0 & 18.4 & 102.3 & -  & 145.3& 322.9 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{Execution time (sec) of 3-FSM in Pangolin (PA) and DistGraph 
(DG) ($sup$: minimum support). 
%The number of frequent patterns (\# FP) is also listed in the third column of each input.
}
\label{tab:3-fsm}
\end{table}

\iffalse
\begin{table}[t]
\footnotesize
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|rrr|rrr|rrr}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Mico} & \multicolumn{3}{c|}{Patent} & \multicolumn{3}{c}{Youtube}          \\ \hline
$sup$ & PA & DG & \# FP & PA & DG & \# FP & PA & DG & \# FP \\ \hline
300  & 3.9 & 52.2 & 5,890 & 14.7 & 19.9 & 21,756 & 96.9 & - & 3,063 \\
500  & 3.6 & 52.9 & 3,639 & 15.8 & 18.7 & 21,480 & 97.7 & - & 2,854 \\
1000 & 3.0 & 59.1 & 1,361 & 18.1 & 18.6 & 20,275 & 98.0 & - & 2,524 \\
5000 & 2.4 & 58.1 & 9    & 27.0 & 18.4 & 5,933  & 102.3& - & 1,487 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{3-FSM performance comparison between Pangolin (PA) and DistGraph 
(DG)~\cite{DistGraph} over Patent with minimum support ($sup$) of 300, 500, 1K and 5K. 
The number of frequent patterns (\# FP) is also listed in the third column
of each input.}
\label{tab:3-fsm}
\end{table}
\fi


==> sections/tbl_4fsm.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|rrr}
\Xhline{2\arrayrulewidth}
$sup$ & Pangolin & DistGraph \\ \hline
15K   & 438.90   & 129.01 \\
20K   & 224.69   & 81.89  \\
30K   & 31.88    & 26.21  \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{4-FSM performance comparison between Pangolin and DistGraph~\cite{DistGraph}.}
\label{tab:4-fsm}
\end{table}

\iffalse
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|rrr}
\Xhline{2\arrayrulewidth}
$sup$ & Pangolin & DistGraph & \# freq\_patterns \\ 
\hline
15K       & 438.90   & 129.01    & 1,917              \\
20K       & 224.69   & 81.89     & 471               \\
30K       & 31.88    & 26.21     & 68                \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{4-FSM performance comparison between Pangolin and DistGraph~\cite{DistGraph} 
over Patent with minimum support ($sup$) of 10K, 15K, 20K and 30K.}
\label{tab:4-fsm}
\end{table}
\fi


==> sections/tbl_kcl.tex <==
\begin{table}[t]
\footnotesize
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{c|rrrr}
\Xhline{2\arrayrulewidth}
k=4 (28t) & PA-CPU & PA-GPU & KClist \\ \hline
Youtube   &  3.08  & 0.09   & 0.42   \\
LiveJ     & 26.31  & 2.46   & 1.85   \\
Orkut     & 82.29  & 4.65   & 4.11   \\
\Xhline{2\arrayrulewidth}
\end{tabular}
%}
\caption{4-clique performance comparison between Pangolin (PA) and KClist~\cite{KClique}.}
\label{tab:4-clique}
\end{table}

\iffalse
\begin{table}[t]
\footnotesize
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{c|rrrr}
\Xhline{2\arrayrulewidth}
k=4 (28t) & PA-CPU  & PA-GPU & KClist & \# 4-cliques  \\ \hline
Youtube   &  3.08   & 0.09   & 0.42   & 176,614,367   \\
LiveJ     & 26.31   & 2.46   & 1.85   & 9,933,532,019 \\
Orkut     & 82.29   & 4.65  & 4.11   & 3,221,946,137 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
%}
\caption{4-clique performance comparison between Pangolin (PA) and KClist~\cite{KClique}. The number of 4-cliques are also listed.}
\label{tab:4-clique}
\end{table}
\fi


==> sections/tbl_motif.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|rrr}
\Xhline{2\arrayrulewidth}
k=4     & \bf{PA-CPU}  & \bf{PA-GPU} & \bf{PGD}   \\ \hline
Mico    & 175.56  & 5.33   & 1.23  \\
Patent  & 209.07  & 4.41   & 6.69  \\
Youtube & 4405.32 & -      & 40.60 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{4-motif performance comparison between Pangolin (PA) and PGD~\cite{PGD}.}
\label{tab:4-motif}
\end{table}


==> sections/tbl_opt.tex <==
\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
\iffalse
\begin{table}[]
	\resizebox{0.49\textwidth}{!}{
	\begin{tabular}{|c|c|c|c|c|c|}
	\hline
    & \thead{DAG} & \thead{Eager\\ Prune} & \thead{Customized\\ Pattern} & \thead{Inspection\\Exection}  & \thead{Scalable\\ allocator} \\ \hline
	TC  & \checkmark &            &            & \checkmark  &   \\ \hline
	CF  & \checkmark & \checkmark &            & \checkmark  &   \\ \hline
	MC  &     &      & \checkmark & \checkmark &                 \\ \hline
	FSM &     &      & \checkmark & \checkmark & \checkmark      \\ \hline
\end{tabular}
}
\vspace{0.1cm}
\caption{Optimizations enabled in each application.}
%\vspace{0.6cm}
\label{tab:opt}
\end{table}
\fi

\begin{table}[t]
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{c|cccc}
			\Xhline{2\arrayrulewidth}
			\hline
      \thead{Applications}	& \thead{DAG} & \thead{Eager Prune} & \thead{Memorization} & \thead{Customized Pattern} \\ \hline
			TC  & \checkmark &            &            &            \\ %\hline
			CF  & \checkmark & \checkmark &            &            \\ %\hline
			MC  &            &            & \checkmark & \checkmark \\ %\hline
			FSM &            &            & \checkmark & \checkmark \\ %\hline
			\Xhline{2\arrayrulewidth}
		\end{tabular}
	}
	\vspace{0.1cm}
	\caption{Optimizations enabled in each application.}
	\vspace{-0.1cm}
	\label{tab:opt}
\end{table}


==> sections/tbl_tc.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|rrrrr}
\Xhline{2\arrayrulewidth}
Input   & \bf{PA-CPU} & \bf{PA-GPU} & \bf{GAP} & \bf{Arabesque} & \bf{RStream} \\ \hline
LiveJ   & 0.59  & 0.055   & 0.47  & 313.53 & 610.28   \\
Orkut   & 3.88  & 0.24   & 4.17  & 1336.22 & 759.34   \\
Twitter & 38.83 & 2.92   & 40.11 & - & - \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Execution time (sec) of TC in Pangolin (PA) and 
GAP.}
\label{tab:tc}
\end{table}

\iffalse
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|rrrr}
\Xhline{2\arrayrulewidth}
(sec)   & PA-CPU& PA-GPU & GAPBS & \# triangles \\ \hline
LiveJ   & 0.59  & 0.17 & 0.47  & 285,730,264     \\
Orkut   & 3.88  & 0.69 & 4.17  & 627,584,181     \\
Twitter & 38.83 & 8.13 & 40.11 & 17,295,646,010  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Triangle counting performance comparison between Pangolin (PA) and 
GAPBS~\cite{GAPBS}. Triangle counts are also listed.}
\label{tab:tc}
\end{table}
\fi

